The Flood Mitigation Problem in a Road Network

Natural disasters are highly complex and unpredictable. However, long-term planning and preparedness activities can help to mitigate the consequences and reduce the damage. For example, in cities with a high risk of flooding, appropriate roadway mitigation can help reduce the impact of floods or high waters on transportation systems. Such communities could benefit from a comprehensive assessment of mitigation on road networks and identification of the best subset of roads to mitigate. In this study, we address a pre-disaster planning problem that seeks to strengthen a road network against flooding. We develop a network design problem that maximizes the improvement in accessibility and travel times between population centers and healthcare facilities subject to a given budget. We provide techniques for reducing the problem size to help make the problem tractable. We use cities in the state of Iowa in our computational experiments.

==> companion.tex <==
%
%%\appendix
%%\makeatletter
%%\@addtoreset{equation}{section}
%%\makeatother
%%\setcounter{secnumdepth}{0}
%%\renewcommand{\theequation}{C.\arabic{equation}}
%%\renewcommand{\theequation}{C.\arabic{equation}}
%\section*{Appendices}
%\addcontentsline{titletoc}{section}{Appendices}
%\renewcommand{\thesubsection}{\Alph{subsection}}
%\renewcommand*{\thesection}{\appendixname~\Alph{section}}
%
%
%\section{Detailed results for the case study} \label{Ap-results}
%
%\begin{table}[!ht]
%	%	\small
%	\renewcommand{\arraystretch}{1}
%	\centering
%	\caption{Results of the case study for $p=24$}
%	\begin{adjustbox}{max width=\textwidth}	
%    \begin{tabular}{lclrrrrcc}
%	\toprule
%	Instance & \# HCFs & Capacity & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{ Obj } & \multicolumn{1}{c}{Ext} & \# upgraded roads & Length of upgrades (mi) \\
%	\midrule
%	1     & 3     & Identical & 15\%  & 5.0\% &    118,777  &          1,444  & 32    & 10.96 \\
%	2     & 3     & Identical & 15\%  & 7.5\% &    117,436  &             103  & 57    & 18.75 \\
%	3     & 3     & Identical & 15\%  & 10.0\% &    117,346  &                13  & 75    & 24.22 \\
%	4     & 3     & Identical & 15\%  & 15.0\% &    117,333  &                  0  & 76    & 26.40 \\
%	5     & 3     & Identical & 30\%  & 5.0\% &    118,745  &          1,806  & 32    & 10.96 \\
%	6     & 3     & Identical & 30\%  & 7.5\% &    117,042  &             103  & 51    & 17.80 \\
%	7     & 3     & Identical & 30\%  & 10.0\% &    116,939  &                  0  & 75    & 24.22 \\
%	8     & 3     & Identical & 30\%  & 15.0\% &    116,939  &                  0  & 75    & 24.22 \\
%	9     & 3     & Different & 15\%  & 5.0\% &    128,066  &          1,575  & 32    & 11.02 \\
%	10    & 3     & Different & 15\%  & 7.5\% &    127,180  &             688  & 51    & 18.03 \\
%	11    & 3     & Different & 15\%  & 10.0\% &    126,527  &                36  & 57    & 20.81 \\
%	12    & 3     & Different & 15\%  & 15.0\% &    126,493  &                  2  & 75    & 24.59 \\
%	13    & 3     & Different & 30\%  & 5.0\% &    126,584  &          1,586  & 35    & 11.14 \\
%	14    & 3     & Different & 30\%  & 7.5\% &    125,667  &             669  & 52    & 18.03 \\
%	15    & 3     & Different & 30\%  & 10.0\% &    125,038  &                40  & 55    & 20.90 \\
%	16    & 3     & Different & 30\%  & 15.0\% &    124,998  &                  0  & 76    & 25.08 \\
%	17    & 7     & Identical & 15\%  & 5.0\% &      69,257  &             191  & 36    & 11.66 \\
%	18    & 7     & Identical & 15\%  & 7.5\% &      69,074  &                  7  & 62    & 18.55 \\
%	19    & 7     & Identical & 15\%  & 10.0\% &      69,066  &                  0  & 66    & 21.22 \\
%	20    & 7     & Identical & 15\%  & 15.0\% &      69,066  &                  0  & 66    & 21.22 \\
%	21    & 7     & Identical & 30\%  & 5.0\% &      67,445  &             189  & 36    & 11.58 \\
%	22    & 7     & Identical & 30\%  & 7.5\% &      67,263  &                  7  & 62    & 18.55 \\
%	23    & 7     & Identical & 30\%  & 10.0\% &      67,257  &                  0  & 66    & 21.22 \\
%	24    & 7     & Identical & 30\%  & 15.0\% &      67,257  &                  1  & 65    & 21.22 \\
%	25    & 7     & Different & 15\%  & 5.0\% &    111,524  &          1,583  & 33    & 11.14 \\
%	26    & 7     & Different & 15\%  & 7.5\% &    110,643  &             702  & 51    & 18.29 \\
%	27    & 7     & Different & 15\%  & 10.0\% &    109,985  &                44  & 55    & 20.78 \\
%	28    & 7     & Different & 15\%  & 15.0\% &    109,944  &                  2  & 76    & 25.05 \\
%	29    & 7     & Different & 30\%  & 5.0\% &    107,835  &          1,578  & 33    & 11.14 \\
%	30    & 7     & Different & 30\%  & 7.5\% &    106,950  &             693  & 51    & 18.09 \\
%	31    & 7     & Different & 30\%  & 10.0\% &    106,293  &                36  & 56    & 20.75 \\
%	32    & 7     & Different & 30\%  & 15.0\% &    106,257  &                  0  & 75    & 24.59 \\
%	\bottomrule
%\end{tabular}%
%	\end{adjustbox}
%	\label{p24}%
%\end{table}%
%
%
%
%
%\begin{table}[!ht]
%	%	\small
%	\renewcommand{\arraystretch}{1}
%	\centering
%	\caption{Results of the case study for $p=18$}
%	\begin{adjustbox}{max width=\textwidth}	
%    \begin{tabular}{lclrrrrcc}
%	\toprule
%	Instance & \# HCFs & Capacity & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{ Obj } & \multicolumn{1}{c}{ETT} & \# upgraded roads & Length of upgrades (mi) \\
%	\midrule
%	33    & 3     & Identical & 15\%  & 5.0\% &    127,898  &          2,021  & 33    & 11.05 \\
%	34    & 3     & Identical & 15\%  & 7.5\% &    126,023  &             145  & 54    & 18.12 \\
%	35    & 3     & Identical & 15\%  & 10.0\% &    125,889  &                11  & 81    & 25.31 \\
%	36    & 3     & Identical & 15\%  & 15.0\% &    125,878  &                  0  & 84    & 28.45 \\
%	37    & 3     & Identical & 30\%  & 5.0\% &    127,898  &          2,340  & 33    & 11.05 \\
%	38    & 3     & Identical & 30\%  & 7.5\% &    125,758  &             199  & 52    & 17.57 \\
%	39    & 3     & Identical & 30\%  & 10.0\% &    125,559  &                  0  & 81    & 25.31 \\
%	40    & 3     & Identical & 30\%  & 15.0\% &    125,558  &                  0  & 83    & 26.27 \\
%	41    & 3     & Different & 15\%  & 5.0\% &    137,676  &          2,181  & 30    & 10.92 \\
%	42    & 3     & Different & 15\%  & 7.5\% &    136,246  &             750  & 51    & 18.04 \\
%	43    & 3     & Different & 15\%  & 10.0\% &    135,560  &                65  & 54    & 20.71 \\
%	44    & 3     & Different & 15\%  & 15.0\% &    135,495  &                  0  & 82    & 26.52 \\
%	45    & 3     & Different & 30\%  & 5.0\% &    136,185  &          2,272  & 30    & 10.92 \\
%	46    & 3     & Different & 30\%  & 7.5\% &    134,647  &             734  & 51    & 18.04 \\
%	47    & 3     & Different & 30\%  & 10.0\% &    133,987  &                74  & 55    & 20.68 \\
%	48    & 3     & Different & 30\%  & 15.0\% &    133,913  &                  0  & 83    & 27.00 \\
%	49    & 7     & Identical & 15\%  & 5.0\% &      73,926  &             302  & 41    & 11.25 \\
%	50    & 7     & Identical & 15\%  & 7.5\% &      73,640  &                16  & 69    & 18.49 \\
%	51    & 7     & Identical & 15\%  & 10.0\% &      73,624  &                  0  & 76    & 23.64 \\
%	52    & 7     & Identical & 15\%  & 15.0\% &      73,624  &                  0  & 76    & 23.64 \\
%	53    & 7     & Identical & 30\%  & 5.0\% &      72,027  &             314  & 41    & 11.25 \\
%	54    & 7     & Identical & 30\%  & 7.5\% &      71,731  &                18  & 64    & 18.44 \\
%	55    & 7     & Identical & 30\%  & 10.0\% &      71,713  &                  0  & 77    & 23.79 \\
%	56    & 7     & Identical & 30\%  & 15.0\% &      71,713  &                  0  & 76    & 23.79 \\
%	57    & 7     & Different & 15\%  & 5.0\% &    120,316  &          2,492  & 31    & 10.92 \\
%	58    & 7     & Different & 15\%  & 7.5\% &    118,590  &             766  & 52    & 18.07 \\
%	59    & 7     & Different & 15\%  & 10.0\% &    117,906  &                82  & 56    & 20.60 \\
%	60    & 7     & Different & 15\%  & 15.0\% &    117,826  &                  1  & 84    & 27.07 \\
%	61    & 7     & Different & 30\%  & 5.0\% &    116,321  &          2,442  & 31    & 10.92 \\
%	62    & 7     & Different & 30\%  & 7.5\% &    114,650  &             770  & 52    & 18.07 \\
%	63    & 7     & Different & 30\%  & 10.0\% &    113,959  &                80  & 55    & 20.58 \\
%	64    & 7     & Different & 30\%  & 15.0\% &    113,885  &                  6  & 82    & 26.52 \\
%	\bottomrule
%\end{tabular}%
%	\end{adjustbox}
%	\label{p18}%
%\end{table}%
%
%\begin{table}[!ht]
%	%	\small
%	\renewcommand{\arraystretch}{1}
%	\centering
%	\caption{Results of the case study for $p=14$}
%	\begin{adjustbox}{max width=\textwidth}	
%    \begin{tabular}{lclrrrrcc}
%	\toprule
%	Instance & \# HCFs & Capacity & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{ Obj } & \multicolumn{1}{c}{ETT} & \# upgraded roads & Length of upgrades (mi) \\
%	\midrule
%	65    & 3     & Identical & 15\%  & 5.0\% &    140,164  &          5,116  & 38    & 11.76 \\
%	66    & 3     & Identical & 15\%  & 7.5\% &    135,313  &             265  & 53    & 17.61 \\
%	67    & 3     & Identical & 15\%  & 10.0\% &    135,087  &                39  & 80    & 24.16 \\
%	68    & 3     & Identical & 15\%  & 15.0\% &    135,048  &                  0  & 94    & 30.27 \\
%	69    & 3     & Identical & 30\%  & 5.0\% &    140,048  &          5,334  & 38    & 11.76 \\
%	70    & 3     & Identical & 30\%  & 7.5\% &    135,112  &             399  & 53    & 17.61 \\
%	71    & 3     & Identical & 30\%  & 10.0\% &    134,733  &                20  & 78    & 24.13 \\
%	72    & 3     & Identical & 30\%  & 15.0\% &    134,714  &                  0  & 90    & 28.09 \\
%	73    & 3     & Different & 15\%  & 5.0\% &    150,323  &          5,238  & 36    & 11.66 \\
%	74    & 3     & Different & 15\%  & 7.5\% &    146,105  &          1,020  & 51    & 17.03 \\
%	75    & 3     & Different & 15\%  & 10.0\% &    145,292  &             207  & 52    & 19.84 \\
%	76    & 3     & Different & 15\%  & 15.0\% &    145,086  &                  0  & 89    & 28.33 \\
%	77    & 3     & Different & 30\%  & 5.0\% &    149,050  &          5,642  & 36    & 11.69 \\
%	78    & 3     & Different & 30\%  & 7.5\% &    144,395  &             986  & 53    & 17.26 \\
%	79    & 3     & Different & 30\%  & 10.0\% &    143,596  &             187  & 55    & 20.17 \\
%	80    & 3     & Different & 30\%  & 15.0\% &    143,409  &                  0  & 90    & 28.81 \\
%	81    & 7     & Identical & 15\%  & 5.0\% &      79,157  &             733  & 45    & 11.34 \\
%	82    & 7     & Identical & 15\%  & 7.5\% &      78,450  &                26  & 70    & 18.34 \\
%	83    & 7     & Identical & 15\%  & 10.0\% &      78,424  &                  0  & 82    & 25.22 \\
%	84    & 7     & Identical & 15\%  & 15.0\% &      78,424  &                  0  & 82    & 25.22 \\
%	85    & 7     & Identical & 30\%  & 5.0\% &      76,918  &             510  & 46    & 11.41 \\
%	86    & 7     & Identical & 30\%  & 7.5\% &      76,439  &                31  & 70    & 18.34 \\
%	87    & 7     & Identical & 30\%  & 10.0\% &      76,409  &                  0  & 81    & 25.22 \\
%	88    & 7     & Identical & 30\%  & 15.0\% &      76,409  &                  0  & 82    & 25.22 \\
%	89    & 7     & Different & 15\%  & 5.0\% &    132,894  &          6,527  & 36    & 11.69 \\
%	90    & 7     & Different & 15\%  & 7.5\% &    127,423  &          1,056  & 52    & 16.93 \\
%	91    & 7     & Different & 15\%  & 10.0\% &    126,687  &             321  & 61    & 20.68 \\
%	92    & 7     & Different & 15\%  & 15.0\% &    126,367  &                  0  & 89    & 28.39 \\
%	93    & 7     & Different & 30\%  & 5.0\% &    127,338  &          5,121  & 36    & 11.66 \\
%	94    & 7     & Different & 30\%  & 7.5\% &    123,269  &          1,053  & 50    & 16.89 \\
%	95    & 7     & Different & 30\%  & 10.0\% &    122,468  &             251  & 55    & 19.96 \\
%	96    & 7     & Different & 30\%  & 15.0\% &    122,219  &                  2  & 88    & 28.09 \\
%	\bottomrule
%\end{tabular}%
%	\end{adjustbox}
%	\label{p14}%
%\end{table}%
%
%
%
%\begin{table}[!ht]
%	%	\small
%	\renewcommand{\arraystretch}{1}
%	\centering
%	\caption{Results of the case study for $p=9$}
%	\begin{adjustbox}{max width=\textwidth}	
%    \begin{tabular}{lclrrrrcc}
%	\toprule
%	Instance & \# HCFs & Capacity & \multicolumn{1}{c}{$\alpha$} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{ Obj } & \multicolumn{1}{c}{ETT} & \# upgraded roads & Length of upgrades (mi) \\
%	\midrule
%	97    & 3     & Identical & 15\%  & 5.0\% &    150,547  &          7,784  & 44    & 11.67 \\
%	98    & 3     & Identical & 15\%  & 7.5\% &    143,227  &             464  & 61    & 17.30 \\
%	99    & 3     & Identical & 15\%  & 10.0\% &    142,805  &                42  & 80    & 24.02 \\
%	100   & 3     & Identical & 15\%  & 15.0\% &    142,763  &                  0  & 97    & 31.48 \\
%	101   & 3     & Identical & 30\%  & 5.0\% &    150,349  &          7,943  & 44    & 11.67 \\
%	102   & 3     & Identical & 30\%  & 7.5\% &    142,980  &             575  & 62    & 17.31 \\
%	103   & 3     & Identical & 30\%  & 10.0\% &    142,441  &                35  & 82    & 24.06 \\
%	104   & 3     & Identical & 30\%  & 15.0\% &    142,405  &                  0  & 96    & 29.30 \\
%	105   & 3     & Different & 15\%  & 5.0\% &    161,450  &          8,088  & 45    & 11.49 \\
%	106   & 3     & Different & 15\%  & 7.5\% &    154,572  &          1,210  & 56    & 15.01 \\
%	107   & 3     & Different & 15\%  & 10.0\% &    153,734  &             372  & 61    & 20.60 \\
%	108   & 3     & Different & 15\%  & 15.0\% &    153,362  &                  0  & 96    & 29.95 \\
%	109   & 3     & Different & 30\%  & 5.0\% &    160,248  &          8,659  & 45    & 11.49 \\
%	110   & 3     & Different & 30\%  & 7.5\% &    152,792  &          1,203  & 61    & 18.03 \\
%	111   & 3     & Different & 30\%  & 10.0\% &    151,943  &             354  & 61    & 19.72 \\
%	112   & 3     & Different & 30\%  & 15.0\% &    151,593  &                  4  & 97    & 30.35 \\
%	113   & 7     & Identical & 15\%  & 5.0\% &      84,455  &             998  & 52    & 11.11 \\
%	114   & 7     & Identical & 15\%  & 7.5\% &      83,521  &                64  & 69    & 18.24 \\
%	115   & 7     & Identical & 15\%  & 10.0\% &      83,464  &                  6  & 88    & 25.77 \\
%	116   & 7     & Identical & 15\%  & 15.0\% &      83,458  &                  0  & 93    & 29.19 \\
%	117   & 7     & Identical & 30\%  & 5.0\% &      82,138  &             813  & 51    & 10.98 \\
%	118   & 7     & Identical & 30\%  & 7.5\% &      81,389  &                64  & 69    & 18.25 \\
%	119   & 7     & Identical & 30\%  & 10.0\% &      81,331  &                  6  & 88    & 25.77 \\
%	120   & 7     & Identical & 30\%  & 15.0\% &      81,325  &                  0  & 92    & 29.04 \\
%	121   & 7     & Different & 15\%  & 5.0\% &    141,853  &          8,256  & 44    & 11.41 \\
%	122   & 7     & Different & 15\%  & 7.5\% &    134,844  &          1,247  & 58    & 17.84 \\
%	123   & 7     & Different & 15\%  & 10.0\% &    133,974  &             378  & 60    & 20.52 \\
%	124   & 7     & Different & 15\%  & 15.0\% &    133,600  &                  3  & 89    & 29.14 \\
%	125   & 7     & Different & 30\%  & 5.0\% &    136,844  &          7,619  & 44    & 11.38 \\
%	126   & 7     & Different & 30\%  & 7.5\% &    130,465  &          1,240  & 58    & 17.84 \\
%	127   & 7     & Different & 30\%  & 10.0\% &    129,606  &             381  & 61    & 20.62 \\
%	128   & 7     & Different & 30\%  & 15.0\% &    129,225  &                  0  & 93    & 29.21 \\
%	\bottomrule
%\end{tabular}%
%	\end{adjustbox}
%	\label{p9}%
%\end{table}%
%
%\newpage
%
%
%
%
%%the number of upgraded roads is almost the same for all types of roads except the residential ones.
%
%%\textbf{Insight:} 
%
%\section{Sensitivity analysis of the covered population}\label{pop_anals}
%The total length and number of times that each type of road has been upgraded over each $p$ value is presented in the first four rows of Table \ref{rtype_p}. The fifth row shows that for covering larger populations, more (miles of) residential roads need to be upgraded. However, the number of upgraded segments among the other types of roads and the number of upgraded roads containing bridges (last row) are almost insensitive to the percentage of the covered population. Table \ref{p_priority} in Section \ref{high} lists the roads with the 100\% frequency for each subset of instances with a specific $p$ value. In total, the number of upgraded roads with 100\% frequency where $p=$ 24, 18, 14, and 9 is equal to 9, 9, 12, and 14 roads, respectively. This
%%We can see that for covering larger populations, more roads with 100\% frequency are upgraded, 
%indicates that for covering larger populations more upgraded roads are needed to connect the OD pairs.
%
%\begin{table}[htbp]
%	\centering
%	\caption{The number and length of the upgraded roads over different $p$ values}
%	\begin{tabular}{llrrrrrrrrrrr}
%		\toprule
%		&       & \multicolumn{2}{c}{p=24} &       & \multicolumn{2}{c}{p=18} &       & \multicolumn{2}{c}{p=14} &       & \multicolumn{2}{c}{p=9} \\
%		\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}    Type  &       & roads & miles &       & roads & miles &       & roads & miles &       & roads & miles \\
%		\midrule
%		Primary &       & 13    &      73,755  &       & 13    &      72,258  &       & 13    &      69,413  &       & 13    &      64,270  \\
%		Secondary &       & 17    &      83,812  &       & 18    &      81,599  &       & 18    &      74,123  &       & 18    &      66,276  \\
%		Tertiary &       & 12    &      68,042  &       & 15    &      69,933  &       & 13    &      68,354  &       & 18    &      73,050  \\
%		Residential &       & 66    &    144,768  &       & 81    &    162,844  &       & 91    &    191,258  &       & 104   &    222,229  \\
%		Total &       & 108   &    370,377  &       & 127   &    386,634  &       & 135   &    403,148  &       & 153   &    425,825  \\
%		\multicolumn{2}{l}{Roads with bridge} & 16    &      70,855  &       & 16    &      68,798  &       & 16    &      64,971  &       & 18    &      68,681  \\
%		\bottomrule
%	\end{tabular}%
%	\label{rtype_p}%
%\end{table}%

